Assimilation of Satellite Active Fires Data

Wildland fires pose an increasingly serious problem in our society. The number and severity of these fires has been rising for many years. Wildfires pose direct threats to life and property as well as threats through ancillary effects like reduced air quality. The aim of this thesis is to develop techniques to help combat the impacts of wildfires by improving wildfire modeling capabilities by using satellite fire observations. Already much work has been done in this direction by other researchers. Our work seeks to expand the body of knowledge using mathematically sound methods to utilize information about wildfires that considers the uncertainties inherent in the satellite data. In this thesis we explore methods for using satellite data to help initialize and steer wildfire simulations. In particular, we develop a method for constructing the history of a fire, a new technique for assimilating wildfire data, and a method for modifying the behavior of a modeled fire by inferring information about the fuels in the fire domain. These goals rely on being able to estimate the time a fire first arrived at every location in a geographic region of interest. Because detailed knowledge of real wildfires is typically unavailable, the basic procedure for developing and testing the methods in this thesis will be to first work with simulated data so that the estimates produced can be compared with known solutions. The methods thus developed are then applied to real-world scenarios. Analysis of these scenarios shows that the work with constructing the history of fires and data assimilation improves improves fire modeling capabilities. The research is significant because it gives us a better understanding of the capabilities and limitations of using satellite data to inform wildfire models and it points the way towards new avenues for modeling fire behavior.

==> body.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Body}\label{sec:body}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




==> ch02/wildfires.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Wildifires}\label{sec:wildfires}
This section section briefly describes the phenomena of wildfires and their impacts on society and the environment.

%\begin{itemize}
%\item Basics of wildland fires.
%\item Properties of fires that are of interest. Fire arrival time, smoke output, burn area, effects on weather.
%\end{itemize}

\subsection{Wildland Fires}
Describing the basic of wildland fire for those who need some background in the subject for further reading. Stress the following:
\begin{itemize}
\item Weather
\item Terrain
\item Fuel
\item General behavior of fires with mention about what can be modeled in the WRF-SFIRE system.
\end{itemize}

\begin{figure}[!ht]
\centering
\includegraphics[width=0.30\textwidth]{fire_triangle.png}
\caption[The fire behavior triangle]{The fire behavior triangle. Weather, fuels, and the terrain are the three biggest factors affecting the behavior of wildfires.}
\label{fig:fire_triangle}
\end{figure}





%Kochanski-2014-APF
%Air pollution forecasting by coupled atmosphere-fire model {WRF} and {SFIRE} with {WRF-Chem}

%Kochanski-2019-MWS,
%Modeling Wildfire Smoke Feedback Mechanisms Using a Coupled Fire-Atmosphere Model With a Radiatively Active Aerosol Scheme




==> ch03/limitations.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Data Limitations}\label{sec:data_limits}

\subsection{Dependence of observations}
The weighting function implies that not all active fire detections are independent. A hot fire near the edge of a pixel can make two fire detections be recorded.

\subsection{False Positives}
Because of a false-positive rate, the log-likelihood eventually flattens out. This is a drawback for various optimization techniques.


==> ch07/assimilate.tex <==
\section{Data Assimilation}
\label{sec:estimate_work}

==> env/pythonenv.tex <==

\usepackage[utf8]{inputenc}

% Default fixed font does not support bold face
\DeclareFixedFont{\ttb}{T1}{txtt}{bx}{n}{8} % for bold
\DeclareFixedFont{\ttm}{T1}{txtt}{m}{n}{8}  % for normal

% Custom colors
\usepackage{color}
\definecolor{deepblue}{rgb}{0,0,0.5}
\definecolor{deepred}{rgb}{0.6,0,0}
\definecolor{deepgreen}{rgb}{0,0.5,0}

\usepackage{listings}

% Python style for highlighting
\newcommand\pythonstyle{\lstset{
language=Python,
basicstyle=\ttm,
otherkeywords={self},             % Add keywords here
keywordstyle=\ttb\color{deepblue},
emph={MyClass,__init__},          % Custom highlighting
emphstyle=\ttb\color{deepred},    % Custom highlighting style
stringstyle=\color{deepgreen},
frame=tb,                         % Any extra options here
showstringspaces=false            %
}}


% Python environment
\lstnewenvironment{python}[1][]
{
\pythonstyle
\lstset{#1}
}
{}

% Python for external files
\newcommand\pythonexternal[2][]{{\hbox{
\pythonstyle
\lstinputlisting[#1]{#2}}\vspace{0.25in}}}

% Python for inline
\newcommand\pythoninline[1]{{\pythonstyle\lstinline!#1!}}


==> env2/bashenv.tex <==

\usepackage[utf8]{inputenc}

% Default fixed font does not support bold face
\DeclareFixedFont{\ttbb}{T1}{txtt}{bx}{n}{10} % for bold
\DeclareFixedFont{\ttmm}{T1}{txtt}{m}{n}{10}  % for normal

% Custom colors
\usepackage{color}
\definecolor{deepblue}{rgb}{0,0,0.5}
\definecolor{deepred}{rgb}{0.6,0,0}
\definecolor{deepgreen}{rgb}{0,0.5,0}

\usepackage{listings}

% Bash style for highlighting
\newcommand\bashstyle{\lstset{
language=Bash,
basicstyle=\ttmm,
otherkeywords={self},             % Add keywords here
keywordstyle=\ttbb\color{deepblue},
emph={python},          % Custom highlighting
emphstyle=\ttbb\color{deepred},    % Custom highlighting style
stringstyle=\color{deepgreen},
frame=tb,                         % Any extra options here
showstringspaces=false            %
}}


% Bash environment
\lstnewenvironment{bash}[1][]
{
\bashstyle
\lstset{#1}
}
{}

% Bash for external files
\newcommand\bashexternal[2][]{{\hbox{
\bashstyle
\lstinputlisting[#1]{#2}}\vspace{0.25in}}}

% Bash for inline
\newcommand\bashinline[1]{{\bashstyle\lstinline!#1!}}


==> env2/newcommands.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% newcommands.tex
% itemize with the explaining text left justified afer the item
% Example:
%   \itembox{CNR} The Control net reduction
%   \itembox{A} Another item
% renders as
% * CNR   The Control net reduction
% * A     Another item
\newcommand{\itembox}[1]{\item {\makebox[0.25in]{#1 \hfill}}}

% Abbreviations
\newcommand{\ie}{{\itshape i.e.}}
\newcommand{\eg}{{\itshape e.g.}}

% Bold symbols
\newcommand{\bs}[1]{\boldsymbol{#1}}

% Cardinality
\newcommand{\card}[1]{n\left(#1\right)} %{\left|#1\right|}
\newcommand{\set}[1]{\left\{#1\right\}}
\newcommand{\nullset}{\varnothing}

% Math Operators
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argmax}{arg\,max}
\newcommand{\abs}[1]{\left\vert#1\right\vert}
\newcommand{\norm}[1]{\left\Vert#1\right\Vert}
\newcommand{\mat}[2]{\left[\begin{array}{#1}#2\\ \end{array}\right]}

% Standard Probability
\DeclareMathOperator{\E}{\mathbb{E}}
% Measure
\newcommand{\PP}{\mathbb{P}}
% Density
\newcommand{\pp}{\pi}
% Space of measures/solutions
\newcommand{\PPspace}{\mathcal{P}}


% indices into sets/spaces
\newcommand{\iparam}{i} % index into parameter space (num samples)
\newcommand{\imesh}{h} % index into mesh/model refinement sequence
\newcommand{\iobs}{k} % index into QoI
\newcommand{\idisc}{k} % index into output discretization
\newcommand{\idata}{j} % index into data (target)

% Sets/Spaces
\newcommand{\RR}{\mathbb{R}}
\renewcommand{\NN}{\mathbb{N}}
\newcommand{\OO}{\mathcal{O}} % sets of indices for set-based inversion alg
\renewcommand{\LL}{\mathcal{L}} % transverse parameterization
\newcommand{\VV}{\mathcal{V}} % voronoi
\newcommand{\BB}{\mathcal{B}} % borel

\newcommand{\CC}{\mathcal{C}} % contour symbol
\newcommand{\cborel}{\CC_{\pspace}} % contour sigma algebra
\DeclareMathOperator*{\contourP}{\PP_{\cborel}}

\newcommand{\paramP}{\PP_\pspace}
\newcommand{\dataP}{\observedP}

\newcommand{\nparams}{P}
\newcommand{\RP}{\RR^\nparams} % parameter space dimensions
\newcommand{\nsamps}{N} % num samples

\newcommand{\ndata}{D} % num data points collected for each observable
\newcommand{\RD}{\RR^\ndata} % data space dimensions

% Sample-Based
\newcommand{\nobs}{O} % number of observables
\newcommand{\RO}{\RR^\nobs} % qoi data space dimensions

% Set-Based
\newcommand{\ndiscs}{M} % number of cells used to discretize data space

\newcommand{\sa}{\sigma\text{-algebra}}
\newcommand{\Chi}{\mbox{\LARGE$\chi$}}

\newcommand{\Rho}{\mbox{\LARGE$\rho$}}
\newcommand{\Nu}{\mbox{\Large$\nu$}}

\newcommand{\true}{\dagger}
% Data-Consistent Inversion Framework
\newcommand{\dimP}{P}
\newcommand{\dimD}{D}
\newcommand{\param}{\lambda}
\newcommand{\paramref}{\param^\true}
\newcommand{\pspace}{{\Lambda}}
\newcommand{\pmeas}{\mu_{\pspace}}
\newcommand{\pborel}{\BB_{\pspace}}
\newcommand{\Pspace}{(\pspace, \pborel, \pmeas)}

\DeclareMathOperator*{\initialP}{\PP_{in}}
\DeclareMathOperator*{\initial}{\pp_{in}}
\DeclareMathOperator*{\updatedP}{\PP_{up}}
\DeclareMathOperator*{\updated}{\pp_{up}}

\DeclareMathOperator*{\obs}{\boldsymbol{o}}
\DeclareMathOperator*{\data}{\boldsymbol{d}}
\newcommand{\dspace}{\mathcal{D}}
\newcommand{\dmeas}{\mu_{\dspace}}
% \newcommand{\dmeas}{\predictedP}
\newcommand{\dborel}{\BB_{\dspace}}
\newcommand{\Dspace}{(\dspace, \dborel, \dmeas)}
\newcommand{\Ospace}{(\dspace, \dborel, \dataP)}

\DeclareMathOperator*{\prior}{\pp_{prior}}
\DeclareMathOperator*{\posterior}{\pp_{post}}

% Labeled QoI maps
\newcommand{\qoiA}{\qoi^{(a)}}
\newcommand{\qoiB}{\qoi^{(b)}}
\newcommand{\qoiC}{\qoi^{(c)}}
\newcommand{\dspaceA}{\dspace_{\qoiA}}
\newcommand{\dspaceB}{\dspace_{\qoiB}}

\newcommand{\qspace}{\mathcal{Q}}
\newcommand{\lam}{\left ( \param \right ) }
\newcommand{\lami}{\left ( \param_\iparam \right ) }
\newcommand{\qoi}{Q}
\newcommand{\q}{q}
\newcommand{\qlam}{\qoi\lam}
\newcommand{\Q}{\left ( \qlam \right )}
\newcommand{\Qi}{\left ( \qoi\lami \right )}
% Model M(u, param) = 0
\newcommand{\M}{\mathcal{M}}

\newcommand{\observedMean}{\mathbf{y}}
\DeclareMathOperator*{\observedP}{\PP_{ob}}
\DeclareMathOperator*{\observed}{\pp_{ob}}
\DeclareMathOperator*{\predictedP}{\PP_{pr}}
\DeclareMathOperator*{\predicted}{\pp_{pr}}

\DeclareMathOperator*{\dciP}{\updatedP = \initialP \frac{\observedP}{\predictedP}}
\DeclareMathOperator*{\dciD}{\updated = \initial \frac{\observed}{\predicted}}
\DeclareMathOperator*{\dci}{\updated\lam = \initial\lam \frac{\observed\Q}{\predicted\Q}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Theorems
\usepackage[english]{babel}
\theoremstyle{plain}
\newtheorem{thm}{Theorem}[section]
\newtheorem{cor}{Corollary}
\newtheorem{lem}{Lemma}
\newtheorem{prop}{Proposition}

\theoremstyle{definition}
\newtheorem{defn}{Definition}
\newtheorem{assumption}{Assumption}[section]

\theoremstyle{remark}
\newtheorem{rem}{Remark}

\theoremstyle{definition}
\newtheorem{ex}{Example}
\numberwithin{equation}{section}
\newtheorem{prob}{Problem}
\numberwithin{equation}{section}
\newtheorem{corollary}{Corollary}[section]



%%% stuff from proposal to sort out later %%%
\newcommand{\sett}[3]{\left\{#1\right\}_{#2}^{#3}}
\newcommand{\supp}{\text{supp}}
\newcommand{\eps}{\varepsilon}
\newcommand{\mbf}[1]{\mathbf{#1}}

\newcommand{\updatedPxN}{\PP_{\text{up},\nsamps}}
\newcommand{\updatedPxNN}{\PP_{\text{up},\bar{\nsamps}}}
\newcommand{\updatedPxM}{\PP_{\text{up},\ndiscs}}
\newcommand{\updatedPxNM}{\PP_{\text{up},\nsamps,\ndiscs}}
\newcommand{\updatedPxNMh}{\PP_{\text{up},\nsamps,\ndiscs,\imesh}}

%%% stuff from mud paper %%% -- commented out means already defined!
\newcommand{\initialCov}{\Sigma_\text{init}}
\newcommand{\observedCov}{\Sigma_\text{obs}}
\newcommand{\predictedCov}{\Sigma_\text{pred}}
\newcommand{\updatedCov}{\Sigma_\text{up}}
\newcommand{\initialMean}{\param_0}
% \newcommand{\observedMean}{\yobs}

\newcommand{\mudpt}{\param^{\text{MUD}}}

% siam cls includes this...
\newtheorem{definition}{Definition}[section]

% subfigure
\newcommand{\subf}[2]{%
  {\small\begin{tabular}[t]{@{}c@{}}
  #1\\#2
  \end{tabular}}%
}


==> env2/pythonenv.tex <==

\usepackage[utf8]{inputenc}

% Default fixed font does not support bold face
\DeclareFixedFont{\ttb}{T1}{txtt}{bx}{n}{8} % for bold
\DeclareFixedFont{\ttm}{T1}{txtt}{m}{n}{8}  % for normal

% Custom colors
\usepackage{color}
\definecolor{deepblue}{rgb}{0,0,0.5}
\definecolor{deepred}{rgb}{0.6,0,0}
\definecolor{deepgreen}{rgb}{0,0.5,0}

\usepackage{listings}

% Python style for highlighting
\newcommand\pythonstyle{\lstset{
language=Python,
basicstyle=\ttm,
otherkeywords={self},             % Add keywords here
keywordstyle=\ttb\color{deepblue},
emph={MyClass,__init__},          % Custom highlighting
emphstyle=\ttb\color{deepred},    % Custom highlighting style
stringstyle=\color{deepgreen},
frame=tb,                         % Any extra options here
showstringspaces=false            %
}}


% Python environment
\lstnewenvironment{python}[1][]
{
\pythonstyle
\lstset{#1}
}
{}

% Python for external files
\newcommand\pythonexternal[2][]{{\hbox{
\pythonstyle
\lstinputlisting[#1]{#2}}\vspace{0.25in}}}

% Python for inline
\newcommand\pythoninline[1]{{\pythonstyle\lstinline!#1!}}


==> env2/usepackages.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% usepackages.tex
% ----------------------------------------------------------------------------- %
% a list of packages I commonly use in my LaTeX deliverables.
\usepackage[T1]{fontenc}
\usepackage[utf8]{inputenc}
\usepackage{textcomp}
\usepackage{floatrow}
\usepackage{url}
\usepackage{paralist}
\usepackage{xparse}
% \usepackage{enumitem}
\usepackage[ruled, vlined]{env/algorithm2e}
% source: https://ctan.org/tex-archive/macros/latex/contrib/algorithm2e/tex

%% Using ragged2e package to get left-justified, ragged-right text throughout body
\usepackage[document]{ragged2e}
\RaggedRight
\setlength{\RaggedRightParindent}{0.5in}
\emergencystretch 1em
\usepackage{etoolbox}
\AtBeginEnvironment{figure}{\setlength{\RaggedRightParindent}{0in}}
\AtBeginEnvironment{table}{\setlength{\RaggedRightParindent}{0in}}
\AtBeginEnvironment{algorithm}{\setlength{\RaggedRightParindent}{0in}}

% ----------------------------------------------------------------------------- %
% Float setup
\usepackage{placeins}
\usepackage{ctable}
\floatsetup[table]{framestyle=colorbox,framefit=yes,heightadjust=all,framearound=all,capposition=top}
\floatsetup[figure]{framestyle=colorbox,framefit=yes,heightadjust=all,framearound=all,capposition=bottom}
\usepackage{caption}
\usepackage{subcaption}

% ---------------------------------------------------------------------------- %
% Bibtex
\usepackage[authoryear]{natbib}

% ---------------------------------------------------------------------------- %
% Math Stuff
\usepackage{amsmath,amssymb,amsfonts,mathrsfs}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% stuff from mud paper
\usepackage{color}
\usepackage{enumerate}

% \usepackage{verbatim,amsmath,amsfonts,epsfig,graphics,setspace,amssymb,
% float,stmaryrd, multirow}
% \usepackage{epsfig}
% \usepackage{placeins}
% \usepackage{enumerate,color}
% \usepackage{url}
% %\usepackage{algorithm}
% %\usepackage{algorithmic}
% %\usepackage[]{algorithm2e}
% \usepackage[lined,ruled]{algorithm2e}
% \input{newcommands}


==> makefile <==
# check for required binaries, fail gracefully with helpful error message.
REQUIRED_BINS := latexmk python
$(foreach bin,$(REQUIRED_BINS),\
    $(if $(shell command -v $(bin) 2> /dev/null),$(info Found `$(bin)`),$(error Please install `$(bin)`)))

# find all files required to compile / files that should trigger an update
CHAPTERS = $(shell find . -type f -name 'chapter*.tex')
APPENDIX = $(shell find . -type f -name 'appendix*.tex')

# changes to images/figures: add/edit this line to reflect your file types
# if you create a new variable (perhaps to track a folder), add it to target 
IMAGES = $(shell find . -type f -name '*.png') 
FIGURES = $(shell find . -type f -name '*.pdf' | grep 'figures')

REFS = $(shell find . -type f -name 'references*.bib')
# custom latex environment/styles for python, bash, etc. (syntax highlighting)
ENVS = $(shell find . -type f -name '*env.tex') 

# file name (without .tex)
FILENAME = dissertation

# dependency list: if changes detected in dependency, rebuild target
TEXFILES := \
	$(FILENAME) \
	abstract \
	notation \
	body \
	env/newcommands \
	env/usepackages \

# adds .tex to path name
TEXS = $(patsubst %, %.tex, $(TEXFILES))

# style-file dependendencies (unlikely to change these, but just in case)
DEPS := \
	ucdDissertation.bst \
	ucdenver-dissertation.cls \

# targets that are labeled as PHONY are treated as always needing an update
# a file doesn't actually need to exist for it to run
.PHONY: all clean examples

# the first real target is the one used when no other arguments are passed to `make`
# by creating a dependency on the pdf, we trigger a compilation by default.
all: $(FILENAME).pdf

# our main target
$(FILENAME).pdf: $(TEXS) $(CHAPTERS) $(APPENDIX) $(REFS) $(IMAGES) $(FIGURES) $(ENVS) $(DEPS)
	latexmk -gg -pdf -bibtex $(FILENAME).tex

examples:
	cd examples && \
	make
	echo "All examples built."

clean:
	latexmk -c $(FILENAME).tex
	/bin/rm -f *.spl
	/bin/rm -f *.bbl
	/bin/rm -f dis*.pdf

sync: all
	git pull
	cp $(FILENAME).bbl output.bbl
	-git commit -a -m sync
	git push github master
	git push overleaf master
	
mac:
	make
	open dissertation.pdf


==> notation.tex <==
\chapter*{\uppercase{Abbreviations and Notation} \label{appendix-notation}}

\section{Abbreviations}

\begin{description}[leftmargin=!,labelwidth=0.5in,font=\normalfont]
	\item
\end{description}


\section{Mathematical Notation}
\begin{description}[leftmargin=!,labelwidth=0.5in,font=\normalfont]
	\item
\end{description}


\subsection{General Notation}

% EDIT BELOW AND REMOVE WHAT YOU DO NOT NEED
\begin{description}[leftmargin=!, labelwidth=0.7in]
  \item[$x$]             italicized, Roman or Greek letter, denotes scalar values
  \item[$\bs{x}$]        italicized, bold, lowercase Roman or Greek letter, denotes a column vector
  \item[$\bs{X}$]        italicized, bold, uppercase Roman or Greek letter, denotes a matrix
	\item[$\bs{X}_{ij}$] 	 denotes the component of matrix $\bs{X}$ occupying row $i$ and column $j$

  \item[$x \in (a, b)$]  the value $x$ is within the interval such that $a < x < b$
  \item[{$x \in (a, b]$}]  the value $x$ is within the interval such that $a < x \leq b$
  \item[$x \in [a, b)$]  the value $x$ is within the interval such that $a \leq x < b$
  \item[{$x \in [a, b]$}]  the value $x$ is within the interval such that $a \leq x \leq b$
  \item[$1_{A}\left(x\right)$] the indicator function,\[1_{A}\left(x \right) = \begin{cases} 1 & x \in A \\ 0 & x \notin A \end{cases}.\]
  \item[$\bs{1}_n$] an column vector of $n$ $1$s
  \item[$\bs{I}$] the identity matrix
  \item[$\bs{I}_n$] the $n \times n$ identity matrix
  \item[$\bs{X}^{-1}$] the inverse matrix, i.e., the operator satisfying $\bs{X}^{-1} \bs{X} = \bs{X} \bs{X}^{-1} = \bs{I}.$
  \item[$\bs{X}^{\top{T}}$] transpose, i.e. the operator satisfying $X_{i,j} = X_{j, i} \; \forall \; i,j \in \mathbb{N}$
  \item[$\otimes$] Kronecker product
  \item[$\odot$] element-wise multiplication
\end{description}

\subsection{Sets}

\begin{description}[leftmargin=!, labelwidth=0.8in]
  \item[$\set{x, y, z, \ldots}$]  the set comprising the elements of $x,$ $y,$ $z,$ $\ldots$
  \item[$\set{x, y, z} \backslash x$]  the set comprising the elements of $y$ and $z$\footnote{In other words, the backslash removes an element (or a subset) from the original set.}
  \item[$\sett{x_i}{i = 1}{n}$]  the set comprising the elements of $x_1, x_2, x_3, \ldots, x_n$
  \item[$\RR$] set of real numbers
	\item[$\NN$] set of natural numbers
  \item[$\bs{x} \in \mathbb{R}^n$] $\bs{x}$ is a vector with $n$ elements, all of which are real numbers
\end{description}

\subsection{Statistical Distributions}
\begin{description}[leftmargin=!, labelwidth=0.8in]
  \item[$\mathcal{N} \left( \mu, \sigma^2 \right)$] the uni-variable Gaussian distribution with mean $\mu$ and variance $\sigma^2$
  \item[$\mathcal{N} \left( \bs{\mu}, \bs{\Sigma} \right)$] the multi-variable Gaussian distribution with mean vector $\bs{\mu}$ and variance-covariance matrix $\bs{\Sigma}$
  \item[$\phi(x)$] the standard Gaussian density function
\end{description}

\subsection{Specialized Notation}
This notation refers to values defined explicitly in the context of this thesis.

\begin{itemize}
\itembox{$\M$} a model that takes input parameters to an (observable) state space
\itembox{$u$} an observable state space from which data is to be collected
\itembox{$\param$} a (model) parameter into model $\M$
\itembox{$\obs$} a Parameter-to-Observables (PtO) map, also denoted $\obs( u\lam )$ or $\obs\lam$, each component of which is a functional  $\obs_i: u\lam \to \RR$ on the observable state\footnote{This map represents performing an individual experiment, which may consist of one or more observations (either in space or time). Arranging observational data into a vector defines the map.}
\itembox{$\qoi$} a Quantity of Interest (QoI) map, also denoted $\qlam$, which acts on observable data to transform the data into a scalar or vector quantity\footnote{For example, it may be the average of measurements encompassed in $\obs$. Technically, this map encompasses the following set of compositions: $Q(\obs(u\lam))$.}
\itembox{$\data$} data representing an individual output of a (possibly vector-valued) QoI map for a particular parameter $\param$, i.e. $\qlam = \data$
\end{itemize}

[TK - add Measure-Theory notation into this section, based on what you have in your newcommands.tex file]

